Styling with Attention to Details

Fashion as characterized by its nature, is driven by style. In this paper, we propose a method that takes into account the style information to complete a given set of selected fashion items with a complementary fashion item. Complementary items are those items that can be worn along with the selected items according to the style. Addressing this problem facilitates in automatically generating stylish fashion ensembles leading to a richer shopping experience for users. Recently, there has been a surge of online social websites where fashion enthusiasts post the outfit of the day and other users can like and comment on them. These posts contain a gold-mine of information about style. In this paper, we exploit these posts to train a deep neural network which captures style in an automated manner. We pose the problem of predicting complementary fashion items as a sequence to sequence problem where the input is the selected set of fashion items and the output is a complementary fashion item based on the style information learned by the model. We use the encoder decoder architecture to solve this problem of completing the set of fashion items. We evaluate the goodness of the proposed model through a variety of experiments. We empirically observe that our proposed model outperforms competitive baseline like apriori algorithm by ~28 in terms of accuracy for top-1 recommendation to complete the fashion ensemble. We also perform retrieval based experiments to understand the ability of the model to learn style and rank the complementary fashion items and find that using attention in our encoder decoder model helps in improving the mean reciprocal rank by ~24. Qualitatively we find the complementary fashion items generated by our proposed model are richer than the apriori algorithm.

==> abstract.tex <==
\begin{abstract}
Fashion as characterized by its nature, is driven by style and trend. Both style and trend carry rich information which is largely unexplored in the context of fashion recommender systems. In this paper, we propose a method that takes into account style and trend information to recommend \textit{complementary} fashion items, given a set of selected fashion items. Complementary items are those items that can be worn along with the selected items according to style and trend. Addressing this problem facilitates in recommending relevant complementary fashion items leading to a richer shopping experience for users. 

Recently, there is a surge of online social websites where fashion enthusiasts post their outfit of the day and other users can like and comment on them. These posts contain a gold-mine of style and trend information. In this paper, we use these posts along with a deep learning based method that learns style and trend information in an automated manner. We pose the problem of predicting complementary fashion items as a machine translation problem where the input is the selected set of fashion items and the output is the fashion item that goes well with them according to the prevailing style and trend. We use the sequence to sequence encoder decoder model to solve this recommendation problem. We evaluate the goodness of the proposed model through a variety of experiments. We empirically observe that our proposed model outperforms competitive baselines like apriori algorithm by \url{~28}\% in terms of accuracy for top-1 recommendation. We generate natural language style-tips for a given query and demonstrate the qualitative results for this task.
\end{abstract}
